Generalized Approximate Message-Passing Decoder for Universal Sparse Superposition Codes

Sparse superposition (SS) codes were originally proposed as a capacity-achieving communication scheme over the additive white Gaussian noise channel (AWGNC) [1]. Very recently, it was discovered that these codes are universal, in the sense that they achieve capacity over any memoryless channel under generalized approximate message-passing (GAMP) decoding [2], although this decoder has never been stated for SS codes. In this contribution we introduce the GAMP decoder for SS codes, we confirm empirically the universality of this communication scheme through its study on various channels and we provide the main analysis tools: state evolution and potential. We also compare the performance of GAMP with the Bayes-optimal MMSE decoder. We empirically illustrate that despite the presence of a phase transition preventing GAMP to reach the optimal performance, spatial coupling allows to boost the performance that eventually tends to capacity in a proper limit. We also prove that, in contrast with the AWGNC case, SS codes for binary input channels have a vanishing error floor in the limit of large codewords. Moreover, the performance of Hadamard-based encoders is assessed for practical implementations.

==> sections/6_Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this work, we have provided an extension of the GAMP algorithm, originally used in compressed sensing, to the vectorial setting that covers SS codes. We have argued that SS codes can be used beyond the scope of the AWGNC and are capacity achieving under GAMP decoding with spatially coupled construction. Furthermore, practical Hadmard operators were used and empirically shown to have similar performance as random operators for large enough section sizes. 
